Generalized Parallel Tempering on Bayesian Inverse Problems

In the current work we present two generalizations of the Parallel Tempering algorithm, inspired by the so-called continuous-time Infinite Swapping algorithm. Such a method, found its origins in the molecular dynamics community, and can be understood as the limit case of the continuous-time Parallel Tempering algorithm, where the (random) time between swaps of states between two parallel chains goes to zero. Thus, swapping states between chains occurs continuously. In the current work, we extend this idea to the context of time-discrete Markov chains and present two Markov chain Monte Carlo algorithms that follow the same paradigm as the continuous-time infinite swapping procedure. We analyze the convergence properties of such discrete-time algorithms in terms of their spectral gap, and implement them to sample from different target distributions. Numerical results show that the proposed methods significantly improve over more traditional sampling algorithms such as Random Walk Metropolis and (traditional) Parallel Tempering.

==> definitions.tex <==
\RequirePackage{amsmath,amsfonts,amssymb}
\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib} %% uncomment this for author-year bibliography
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage{graphicx}
\usepackage{lipsum}
\usepackage{amsfonts,amsmath}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithm}% http://ctan.org/pkg/algorithms
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage{bm}
\usepackage{mathtools}
%declares the bas operator
\usepackage{commath}
%related to the referencing of equations
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{autonum}
%strikout
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage[normalem]{ulem}
\usepackage{multirow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% tiksplotlib            %%
%%									        %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage{pgfplots}
%\DeclareUnicodeCharacter{2212}{−}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}






\newtheorem{assumption}{Assumption}
\newtheorem{thm}{Theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothezis, %%
%% Lemma, Theorem, Proposition              %%
%% use \theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages and macros go here




\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi




%% Here we put definitions and such 
\newcommand{\R}{\mathbb{R}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\vvh}{\mathbf{v}_h}
\newcommand{\uuh}{\mathbf{u}_h}
\newcommand{\xx}{x}
\newcommand{\yy}{y}
\newcommand{\dt}{\Delta t}
\newcommand{\BW}{{\mathcal{B}(W)}}
\newcommand{\BY}{{\mathcal{B}(Y)}}
\newcommand{\fo}{{\mathcal{F}}}
\newcommand{\Dt}{D_{\Delta t}}
\newcommand{\VV}{\mathbf{V}}
\newcommand{\XX}{\mathbf{X}}
\newcommand{\lv}{\left \vert}
\newcommand{\rv}{\right \vert}
\newcommand{\piis}{\overline{\pi}_\mathrm{IS}}
\newcommand{\muis}{\overline{\mu}_\mathrm{IS}}
\newcommand{\lno}{\left \Vert}
\newcommand{\rno}{\right \Vert}
\newcommand{\pil}{\pi_\ell}
\newcommand{\pim}{\pi_{\ell-1}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\eff}{{\mathcal{F}}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\te}{\theta}
\newcommand{\teb}{\bm \theta}
\newcommand{\pib}{\bm \pi}
\newcommand{\mub}{\bm \mu}
\newcommand{\Pw}{{\bm P^\text{(w)}}}
\newcommand{\mubis}{\mub_{\mathrm{W}}}
\newcommand{\phib}{\phi}
\newcommand{\pot}{\Phi(\te;\yy)}
\newcommand{\poth}{\Phi_\ell(\te;\yy)}
\newcommand{\potl}{{\Phi_{\ell-1}(\te;\yy)}}
\newcommand{\zl}{{Z_{\ell-1}}}
\newcommand{\zm}{{Z_{\ell}}}
\newcommand{\potm}{{\Phi_{\ell}(\te;\yy)}}
\newcommand{\dhell}{d_\text{Hell}}
\newcommand{\potp}{\Phi(\te;\yy')}
\newcommand{\work}{\mathcal{W}}
\newcommand{\QoI}{\mathcal{Q}}
\newcommand{\HH}{\mathbf{H}}
\newcommand{\phid}{{\Phi(\theta; y)}}
\newcommand{\sig}{\bm{\sigma}}
\newcommand{\nel}{N_\text{el}}
\newcommand{\ff}{\mathbf{f}}
\newcommand{\Lr}[1]{{\mathcal{L}(L_{r} ( #1 ))}}
\newcommand{\Ls}[1]{{\mathcal{L}(L_{s} ( #1 ))}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\de}{\mathrm{d}}
\newcommand{\alphaq}{\alpha_{\mathrm{swap}}}
\newcommand{\alphaqt}{\alpha_{\mathrm{{swap}}}}
\newcommand{\fbs}{\bar{f}_\sigma}
\newcommand{\yeb}{\bm y}
\newcommand{\fib}{\bm{\varphi}_i}
\newcommand{\psib}{\bm{\psi}_j}
\newcommand{\etab}{\bm{\eta}}
\newcommand{\etabij}{\bm{\eta}_{ij}}
\newcommand{\dij}{\Lambda_{ij}}
\newcommand{\iintx}{\iint_{X^{2K}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  Things for edditing etc
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\newcommand{\ujp}[1]{\color{burgundy}( \textbf{Update}: #1 ) \color{black}} 
\newcommand{\cjp}[2]{{ \color{burgundy}( \textbf{#1}: #2 ) }}   

%%% Defines highlight first_rev
 
\def\Highlight{0}

\ifx\Highlight\undefined
undefed
\else
\if\Highlight1
\newcommand{\rjp}[1]{{\color{orange}#1}}   
\else
\newcommand{\rjp}[1]{{#1}}   
\fi
\fi

 %%% Defines highlight second_rev
 
 \def\HighlightR{0}
 
 \ifx\HighlightR\undefined
 undefed
 \else
 \if\HighlightR1
 \newcommand{\rjpr}[1]{{\color{orange}#1}}   
 \else
 \newcommand{\rjpr}[1]{{#1}}   
 \fi
 \fi

\newcommand{\udjp}[1]{\color{blue}( \textbf{Update}: #1 ) \color{black}}   
\newcommand{\old}[2]{{\color{red}\sout{#1}} {\color{orange} #2}}   

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}
